Forklift: An Extensible Neural Lifter

The escalating demand to migrate legacy software across different Instruction Set Architectures (ISAs) has driven the development of assembly-to-assembly translators to map between their respective assembly languages. However, the development of these tools requires substantial engineering effort. State-of-the-art approaches use lifting, a technique where source assembly code is translated to an architecture-independent intermediate representation (IR) (for example, the LLVM IR) and use a pre-existing compiler to recompile the IR to the target ISA. However, the hand-written rules these lifters employ are sensitive to the particular compiler and optimization level used to generate the code and require significant engineering effort to support each new ISA. We propose Forklift, the first neural lifter that learns how to translate assembly to LLVM IR using a token-level encoder-decoder Transformer. We show how to incrementally add support to new ISAs by fine tuning the assembly encoder and freezing the IR decoder, improving the overall accuracy and efficiency. We collect millions of parallel LLVM IR, x86, ARM, and RISC-V programs across compilers and optimization levels to train Forklift and set up an input/output-based accuracy harness. We evaluate Forklift on two challenging benchmark suites and translate 2.5x more x86 programs than a state-of-the-art hand-written lifter and 4.4x more x86 programs than GPT-4 as well as enabling translation from new ISAs.

==> 2_motivation.tex <==
\section{Error analysis}

\section{Examples/Old motivation}
\label{sec:motivation}

\textbf{should comment examples in story-telling/ASPLOS-style, but being specific too. the samples are attached below, included in
 examples.tex. if you see an error, mention the error (I included error messages)}.


New ISAs are continually being developed,
and existing ISAs continually evolve.  The hardware
accelerator boom has increased the rate at which this
happens, with each new architecture bringing its own
ISA.  This development style puts significant pressure 
on existing programming tools: while in previous eras,
programmer tools could be developed once and not
redeveloped, this is now becoming taxing.  Binary
lifting in particular is a challenging task to implement
by hand, as there is a lot of lost information during
the compilation process that has to be recovered.

New ISAs are continually being developed,
and existing ISAs continually evolve.  The hardware
accelerator boom has increased the rate at which this
happens, with each new architecture bringing its own
ISA.  This development style puts significant pressure 
on existing programming tools: while in previous eras,
programmer tools could be developed once and not
redeveloped, this is now becoming taxing.  Binary
lifting in particular is a challenging task to implement
by hand, as there is a lot of lost information during
the compilation process that has to be recovered.


\subsection{Pitfalls of Hand-Written Lifters}
Hand-written lifters often perform well.  However,
they are sensitive to the particular compiler/optimization
level used to compile the code, as they are specialized
to particular patterns and instructions that
these compiler/optimization levels generate.  An
example is shown in Figure~\ref{fig:LasagneExample},
where Lasagne, which was designed for unoptimized Arm code,
cannot handle various vector instructions.  In contrast,
\name{} is capable of lifting all of this code.

\begin{figure}
    \includegraphics[width=\textwidth]{figures/MotivationDrawingOrig.eps}
    \caption{
    An example of the kinds
    of code that traditional rule-based
    lifters like Lasagne often fail to
    lift.  Here, we have the same
    code that is compiled with two different
    flags, which result in different
    instructions being generated.
    Lasagne, a rule-based lifter
    does not have rules for these
    less frequent instructions that were
    outside the scope of the programs it
    was constructed with in mind.
    \name{} is able to lift these programs
    by simply ensuring that it has some
    training data with the appropriate flags.
    }
    \label{fig:LasagneExample}
\end{figure}

Beyond compiler/optimization level decisions, these
hand-written lifters are architecture-specific.  They
require manually constructed rules, which obviously don't
apply to new architectures.  Worse, the entire process
of rule generation has to be repeated for each architecture,
as engineers for these tools are usually paid by
the companies producing each architecture, so skills in
writing lifters do not accumulate.

\subsection{The Promise of Machine Learning}
Language models promise to overcome this challenge.
Using large datasets like Exebench~\cite{Armengol-Estape2022}, models
can be trained to learn lifting tasks.
%And a number of these models exist~\cite{TODO}.

However, this approach comes with a cost.  In particular,
these models are extremely data-inefficient.  While
a human programmer can build a lifter by constructing
patterns from reference manuals and carefully crafted
examples, existing models require millions of examples.
This comes at a significant compute cost: the model not
only has to be trained, but each example compiled
to the new target.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]
    {figures/ForkliftSystem.eps}
    \caption{Diagram showing how lifelong leraning is used to reduce the computation needed to generate new lifters.}
    \label{ForliftStructure}
\end{figure}

\subsection{Lifelong learning}
Lifelong learning promises a solution to this.
We take advantage of the fact that many ISAs, while
different, share many features and characteristics.
A model that has been trained on one ISA can be
used to learn another ISA far more efficiently.

This is the key concept in \name{}.  An example of this
is shown in Figure~\ref{ForliftStructure}.  Once
\name{} is trained on one architecture, it can be
retrained with significantly lower data costs on
new architectures.





==> analysis.tex <==
\begin{table}
\centering
  \begin{tabular}{l||c|c|c|c|c|c}
    \hline
    \multirow{2}{*}{Lifter} &
      \multicolumn{2}{c}{x86 } &
      \multicolumn{2}{c}{ARM } &
      \multicolumn{2}{c}{RISC-V } \\
      & {Exe} & {Synth} & {Exe} & {Synth} & {Exe} & {Synth} \\
      \hline
      Lasagne & 30.26\% & 37.86\% & 1.03\% & 0.97\% & - & - \\
      ChatGPT & 0.95\% & XX\% & XX\% & XX\% & XX\% & XX\% \\
      \name{} & \textbf{75.56\%} &  \textbf{51.46\%} &  72.37\% & \textbf{69.90\%} & \textbf{72.63\%} & \textbf{83.15\%} \\ \hline
      \end{tabular}    
\caption{\label{tab:summ_results} Result summary. The columns represent accuracy for each ISA on each benchmark set}
\end{table}

==> correlations/correlations_ExeBench_x86_Clang.tex <==
\begin{table}[h]
\centering
\begin{tabular}{
  >{\raggedright}m{2.5cm}
  >{\centering}m{2cm}
  >{\centering}m{2cm}
  >{\centering\arraybackslash}m{2cm}
}
%\rowcolor{white} & \multicolumn{3}{c}{x86\_O3\_Clang} \\
 & Lasagne & GPT4 & Forklift \\
\cellcolor{white}compiles & \cellcolor[HTML]{F5C4AC}0.25 & \cellcolor[HTML]{E36B54}\color{white}0.70 & \cellcolor[HTML]{CC403A}\color{white}0.86 \\
\cellcolor{white}edit\_sim & \cellcolor[HTML]{F5C4AC}0.26 & \cellcolor[HTML]{F6A283}0.46 & \cellcolor[HTML]{F7A688}0.43 \\
\cellcolor{white}c\_length & \cellcolor[HTML]{CEDAEB}-0.10 & \cellcolor[HTML]{BBD1F8}-0.23 & \cellcolor[HTML]{97B8FF}-0.44 \\
\cellcolor{white}n\_fun\_args & \cellcolor[HTML]{F3C8B2}0.22 & \cellcolor[HTML]{BFD3F6}-0.21 & \cellcolor[HTML]{C4D5F3}-0.18 \\
\cellcolor{white}has\_float & \cellcolor[HTML]{E7D7CE}0.08 & \cellcolor[HTML]{DADCE0}-0.02 & \cellcolor[HTML]{D2DBE8}-0.08 \\
\cellcolor{white}has\_strings & \cellcolor[HTML]{E4D9D2}0.05 & \cellcolor[HTML]{D7DCE3}-0.04 & \cellcolor[HTML]{D1DAE9}-0.09 \\
\cellcolor{white}has\_globals & \cellcolor[HTML]{4E68D8}\color{white}-0.87 & \cellcolor[HTML]{EDD2C3}0.14 & \cellcolor[HTML]{D6DCE4}-0.05 \\
\end{tabular}
\caption{ExeBench feature correlations with input/output accuracy, x86, O3, Clang.}
\label{tab:cor_exe_x86_o3_clang}
\end{table}

==> correlations/correlations_Synth_x86_Clang.tex <==
\begin{table}[h]

\centering
\begin{tabular}{l>{\raggedleft}m{2cm}>{\raggedleft\arraybackslash}m{2cm}}
%\rowcolor{white} & \multicolumn{2}{c}{x86\_O3\_Clang} \\
 & Lasagne & Forklift \\
\cellcolor{white}compiles & \cellcolor[HTML]{BE242E}\color{white}0.94 & \cellcolor[HTML]{DA5A49}\color{white}0.77 \\
\cellcolor{white}edit\_sim & \cellcolor[HTML]{F6BFA6}0.29 & \cellcolor[HTML]{F4987A}0.50 \\
\cellcolor{white}c\_length & \cellcolor[HTML]{CAD8EF}-0.14 & \cellcolor[HTML]{ADC9FD}-0.31 \\
\cellcolor{white}n\_fun\_args & \cellcolor[HTML]{A6C4FE}-0.36 & \cellcolor[HTML]{D2DBE8}-0.09 \\
\cellcolor{white}has\_float & \cellcolor[HTML]{CFDAEA}-0.10 & \cellcolor[HTML]{D7DCE3}-0.04 \\
\cellcolor{white}has\_strings & \cellcolor[HTML]{F6BFA6}0.28 & \cellcolor[HTML]{D3DBE7}-0.08 \\
\cellcolor{white}vectorized & \cellcolor[HTML]{6180E9}\color{white}-0.75 & \cellcolor[HTML]{EBD3C6}0.12 \\
\end{tabular}
\caption{Synth feature correlations with input/output accuracy, x86, O3, Clang. GPT-4 is not included as it's close to 0.0 accuracy.}
\label{tab:cor_synth_x86_o3_clang}
\end{table}
